Knowledge is Never Enough: Towards Web Aided Deep Open World Recognition

While today's robots are able to perform sophisticated tasks, they can only act on objects they have been trained to recognize. This is a severe limitation: any robot will inevitably see new objects in unconstrained settings, and thus will always have visual knowledge gaps. However, standard visual modules are usually built on a limited set of classes and are based on the strong prior that an object must belong to one of those classes. Identifying whether an instance does not belong to the set of known categories (i.e. open set recognition), only partially tackles this problem, as a truly autonomous agent should be able not only to detect what it does not know, but also to extend dynamically its knowledge about the world. We contribute to this challenge with a deep learning architecture that can dynamically update its known classes in an end-to-end fashion. The proposed deep network, based on a deep extension of a non-parametric model, detects whether a perceived object belongs to the set of categories known by the system and learns it without the need to retrain the whole system from scratch. Annotated images about the new category can be provided by an 'oracle' (i.e. human supervision), or by autonomous mining of the Web. Experiments on two different databases and on a robot platform demonstrate the promise of our approach.

==> method.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.48\textwidth,height=0.15\textwidth]{imgs/method-owr2-crop.pdf}
 \caption{Overview of the proposed OWR pipeline. Given an input image, the DeepNNO algorithm assigns it a class label. If the object is recognized as novel, the image label is obtained by querying the web. The obtained label is then verified by a human and used to download images for the new semantic category. Finally, the DeepNNO model is incrementally updated by exploiting the downloaded data. % and a memory of relevant old classes, the network is updated and is extended with the class mean of the previously unknown class.
 }
   \label{fig:framework}
\vspace{-19pt}
\end{figure}
%\subsection{Overview}
\vspace{-5pt}
In this section we describe our proposed framework for OWR. Our framework (Fig.~\ref{fig:framework}) contains two core components. The first is an OWR model, named Deep Nearest Non-Outlier (DeepNNO), which merges the NNO classification algorithm with the power of deep representations, within an end-to-end trainable deep architecture (section~\ref{sec:deepnno}). The second is a semi-automatic pipeline based on Web queries (section~\ref{sec:web-download}) which replaces the presence of an oracle giving to the algorithm both labels and data relative to novel classes, as assumed by previous OWR approaches~\cite{bendale2015towards}. %We then introduce the proposed deep learning model for OWR, \textit{i.e.} Deep Nearest Non-Outlier (DeepNNO), which is able to both detect instances of novel classes and incrementally add them to its semantic space. Finally, we show how an OWR system for robotic platforms can be built using Web queries. %(Fig.\ref{fig:framework}).
In the following, we start by formalizing the OWR problem.%, describing previous methods derived by Nearest Class Mean (NCM)~\cite{mensink2012metric}. 
%\massi{In particular, in section \ref{sec:deepnno} we describe the building block of our algorithm, the Deep Nearest Non-Outlier (DeepNNO), a novel deep learning architecture which is able to both detect instances of novel classes and incrementally add them to its semantic space. In section \ref{sec:web-download}, we present a simple framework which allows to automatically collect images of categories unknown to the model by means of Web queries, avoiding the need of an oracle which provides them to the system.} 


\vspace{-4pt}
\subsection{Problem Definition}
\vspace{-5pt}
As stated in Section \ref{sec:intro}, the aim of Open World Recognition is to learn a model able to: (i) correctly classify samples of known classes, 
for which the model has been trained on; (ii) detect instances belonging to novel classes, unseen during training; (iii) incrementally include novel
classes within the set of known ones, extending the capabilities of the classifier.

Formally, let us denote as
$\mathcal{T}_t=\{(x_i,k_i)\}$ the training set, where $x_i$ refers to the $i$-{th} image and $k_i$ its semantic label. %The semantic label 
%Let $k_i \in \mathcal{K}_0$ and $\mathcal{K}_0=\{1,\dots,N\}$ be the set of $N$ $known$ classes. %: we denote $\mathcal{K}$ as the set of \textit{known} classes. 
In OWR the training samples are provided in an incremental fashion, \ie $\mathcal{T}_t$ denotes the training set at time $t$ with cardinality $M_t=|\mathcal{T}_t|$. Furthermore $k_i \in \mathcal{K}_t$ and the set of \emph{known categories} $\mathcal{K}_t$ is dynamically updated. Specifically, this set is initialized considering 
labels associated to the first $N$ semantic categories, \textit{i.e.}  $\mathcal{K}_0=\{1,\dots,N\}$, and it is progressively extended when novel classes are discovered. In summary, we denote the initial set of known classes as $\mathcal{K}_0$ and the set of known classes after $t$ incremental steps as $\mathcal{K}_t$, with $\mathcal{K}_{t}\subset\mathcal{K}_{t+1}$. Similarly let $\mathcal{T}_0$ denote the training set exploited to learn the initial classification model $f$ which is then updated with $\mathcal{T}_t$.%$\phi_\Theta$, where $\Theta$ denotes the model parameters. %for recogniking instances of a class $k \in \mathcal{K_0}$.
%\massi{$\mathcal{T}$ grows???}

In OWR at each time step our goal is twofold. First, we want to detect if a new sample $x_n$ is an instance of a novel class, \ie if the associated label $k_n \in \mathcal{U}_t$, where $\mathcal{U}_t$ is the set of \textit{unknown categories} after $t$ incremental steps. %such that $\mathcal{K}_{t+1}=\mathcal{K}_{t}\cup y_j$. \massi{If a new samples belong %Third, we want to update our training set considering $\mathcal{K}_{t+1}=\mathcal{K}_{t}\cup y_j$.
{Second, %given the semantic label $k^*_j$ of the novel class, 
we want to incrementally update our classification model $f$ such that $\mathcal{K}_{t+1}=\mathcal{K}_{t}\cup \{k_n\}$. %considering the extended training set $\mathcal{T}_{t+1}=\mathcal{T}_t \cup \{ (x_n, k_n) \}$}. %such that $\mathcal{K}_{t+1}=\mathcal{K}_{t}\cup y_j$. \massi{If a new samples belong %Third, we want to update our training set considering $\mathcal{K}_{t+1}=\mathcal{K}_{t}\cup y_j$.
%At deployment time, the robot will encounter instances $x_j \in \mathcal{D}$ \textit{without} any semantic label associated. Differently from standard recognition scenario, the unknown label $y_j$ associated to $x_j$ may belong not only to the set of known classes $\mathcal{K}_t$, but to \textit{any semantic category existing in the real world}. We denote this latter set as $\mathcal{W}$ and we write $y_j \in \mathcal{W}$. Note that $\mathcal{K}_t\subset\mathcal{W}$ and we denote as $\mathcal{U}_t=\mathcal{W}\setminus\mathcal{K}_t$ the set of \textit{unknown} categories after $t$ incremental steps. % \ie the set of \textit{unknown} classes.
In the following we describe the proposed technique to fulfill this goal. 
Before %going into the details of 
detailing our approach, we review the Nearest Class Mean (NCM) \cite{mensink2012metric} algorithm and previous works \cite{bendale2015towards} extending NCM to tackle
the OWR problem.


\vspace{-4pt}
\subsection{From Nearest Class Mean to Nearest Non-Outlier}
\vspace{-4pt}
The NCM algorithm~\cite{mensink2012metric} is a non-parametric classification algorithm which operates in traditional closed world setting (\ie no incremental learning and novel category discovery process take place). NCM computes a mean feature vector for each semantic category and assigns an input image to a class according to the distance between the image and the mean vectors in the feature space. 
Formally, let us denote with $\phi(\cdot)$ a function that, given an image $x$, extracts a feature vector in a $m$-dimensional space. %, \ie $k=f(x)$ with $k\in\Re^m$. 
The NCM algorithm assigns a class label $k^*$ to an input image computing:
\begin{equation}
\label{eq:ncm-prediction}
k^*=\argmin_{k \in \mathcal{K}}d_k(x)=\argmin_{k \in \mathcal{K}} ||\phi(x) - \mu_k ||
\end{equation}
where $\mu_k \in \Re^m$ is the mean feature vector relative to class $k\in \mathcal{K}$ in the training set, and $d_k(x)$ is the distance between 
the mean vector and the features extracted from the input sample. 
%The mean is computed through:
% \begin{equation}
% \mu_j=\frac{1}{|\mathcal{T}_j|}\sum_{x \in \mathcal{T}_j}{f(x)}
% \end{equation} 
% where $\mathcal{T}_j$ denotes the instances of the training set belonging to class $j$.
In \cite{mensink2012metric} the authors proposed to improve the performance of the traditional NCM by including a metric learning procedure. 
In particular, let us suppose to have a matrix $W\in \Re^{m\times d}$ which projects the feature vectors into a $d$-dimensional space. In \cite{mensink2012metric}, Mensink \textit{et al.} proposed to optimize $W$ by minimizing the following loss:
\begin{equation}
\label{eq:loss}
\mathcal{L}=-\frac{1}{M}\sum_{(x_i,k_i)\in \mathcal{T}} \log p_{k_i}(x_i)
\end{equation}
where $p_k(x)= e^{-\frac{1}{2} d_k^W(x)}$, $d_k^W(x) = ||W^T \phi(x) - W^T \mu_k ||$.

%where $W \in \Re^{m\times d}$ is a matrix projecting the feature vectors into %from an $m$-dimensional to 
%a $d$-dimensional space. 
%The matrix $W$ is estimated during training considering the log-likelihood on the training samples.

While NCM is 
%a simple and 
an effective algorithm for addressing visual recognition tasks, it only works under a closed world assumption. To break this assumption, 
Bendale \textit{et al.} \cite{bendale2015towards} extended NCM to OWR settings, presenting the Nearest Non-Outlier algorithm (NNO). %NNO introduces two main modifications into 
%the NCM algorithm. The first is to use 
In NNO for each sample the estimated class distances $d_k^W(x), \ \forall k \in \mathcal{K}_t$, are used to compute a set of class-specific scores defined as: % for each class given by: 
\begin{equation}
\label{eq:nno-score}
s_k(x)=\eta_\tau \left(1-\frac{d_k^W(x)}{\tau}\right)
\end{equation}
where $\tau$ is a user-defined parameter and $\eta_\tau$ is a normalization factor depending on $\tau$. These scores are interpreted as probabilities after applying a clamping function $p_k(x)=\max(0, s_k(x))$. %it possible to obtain a class probability through:
% \begin{equation}
% \label{eq:nno-prob}
% \end{equation}
where a clamping function is introduced as $s_k(x)$ could be negative. 
%In NNO the scores are used also to detect if a sample $x$ belongs to a novel class and the following prediction function is defined:
These probabilities are used to detect if a sample $x$ belongs to a novel class, by defining the following prediction function:
\begin{equation}
\label{eq:nno-prediction}
k^*=\begin{cases}
      u \in \mathcal{U}_t & \text{if}\ 
      p_k(x)=0 \ \ \ \forall k \in \mathcal{K}_t\\
      \argmax_{k\in\mathcal{K}_t} p_k(x) & \text{otherwise}
    \end{cases}
\end{equation}
where a sample belongs to the class $u$ if it is \textit{rejected} (\ie $p_k(x)=0$) by all known classes $k\in\mathcal{K}_t$.
%From these definitions, a sample is rejected by class $j$ if $s_j(x)<0$ and, consequently, a sample belongs to a novel class if $s_j(x)=0 \,\,\forall j \in \mathcal{K}_t$, 
%thus obtain 
%\massi{A sample belongs to hte novel }
In \cite{bendale2015towards} it is assumed that every time a sample is detected as an instance of a novel class, \ie $k^*=u$, an oracle provides the correct label and 
other images for the same class. These images are used to compute the mean feature vector for the novel class
%Furthermore, when $y^*= u$ they also proposed to use some samples of the new class %(given by external sources) 
%to compute a novel class mean vector 
$\mu_u$ which is then included in the classification model. 
%Since in NNO class-specific probability estimates are considered, the optimikation function used to estimate the matrix $W$ is converted to a binary cross-entropy loss. 
In \cite{bendale2015towards} the matrix $W$ is estimated during training minimizing a loss as in Eqn. (\ref{eq:loss}) and then kept fixed during deployment. The parameter $\tau$ is 
obtained through cross-validation. %after training. 
 %$u_t$ which is thus added to the current classification model. %Both $W$ and $\tau$ are kept fixed during deployment and during each incremental step.
 
Previous works ~\cite{bendale2015towards,de2016online} showed how NNO is an effective approach for OWR. However, this method is based on a shallow classification model. Here we demonstrate that the performances of NNO can be significantly boosted through deep architectures. We further show that, by automatically leveraging images from the web, it is possible to 
build a %\massi{maybe one could add an adjective here that gets rid of the need to add something at the end of this sentence. I am thinking "practical" or something like this, to highlight that it works in the wild to use your favorite word ;-)} 
practical OWR systems for visual recognition in robotics platforms, with very limited need of human assistance. %\massi{I think you need to clarify what you mean here, maybe by adding "without the need for human assistance"}. %which avoids any oracle assumption.

\vspace{-5pt}
\subsection{Proposed Method}
\vspace{-5pt}
\subsubsection{DeepNNO}

\label{sec:deepnno}
%In this paper we propose a novel end-to-end deep neural network for OWR derived from NNO, 
The \textit{Deep Nearest Non-Outlier} algorithm is obtained from NNO with the following modifications: (i)
the feature extractor function is replaced with deep representations derived from neural network layers; (ii)
an online update strategy is adopted for the mean vectors $\mu_k$; %, $k \in \mathcal{K}_t$;
(iii) an appropriate loss is optimized %network using the error produced by the current means using standard gradient-based optimization algorithms.
using stochastic gradient descent (SGD) methods in order to %effectively 
compute the feature representations and the associated class specific means.

%\massi{The proposed deep architecture is obtained from NNO with the following modifications: (i)
%the feature extractor function is replaced with deep representations derived from neural network layers; (ii)
%an online update strategy is proposed for the mean vectors $\mu_k$, $k \in \mathcal{K}_t$; % In this case an online or approximate estimate based on the current features can be employed.
%(iii) train the network using the error produced by the current means using standard gradient-based optimization algorithms.}

Inspired by the recent work \cite{guerriero2018deep},
we 
%propose to % I removed this to make it feel less repetitive from above
replace the feature extractor function $\phi(\cdot)$ with deep representations derived from a neural network $\phi_\Theta(x)$
and define the class-specific probability scores as follows:
\begin{equation}
\label{eq:deep-nno-prob}
p_k(x)=\exp\left(-\frac{1}{2}||\phi_\Theta(x) - \mu_k ||\right) .
\end{equation}
Note that, differently from \cite{bendale2015towards}, we do not consider explicitly the matrix $W$ since this is replaced by the network parameters $\Theta$. % is already addressed by training the deep features.
Furthermore, we avoid to use a clamping function as this could hamper the gradient flow within the network. %To obtain a deep version of NNO, first we review the scoring function defined by equation\eqref{eq:nno-prob}. In fact, this function contains a clamping function which 
%could hamper the gradient flow within the network. To this extent we reformulate the scoring function as:
This formulation is similar to the NNO version proposed in \cite{de2016online} which have been showed to be more effective than that in \cite{bendale2015towards} for online scenarios. 

In OWR the classification model must be updated as new samples arrive. In DeepNNO this translates into incrementally updating the feature representations $\phi_\Theta(x)$ and defining an appropriate strategy for updating the class mean vectors. %Following \cite{de2016online}, we propose to dynamically update the class means. 
Given a mini-batch of samples $\mathcal{B}=\{(x_1,k_1),\dots, (x_b,k_b)\}$, we compute the mean vectors through:
\begin{equation}
\label{eq:deep-nno-means}
\mu_k^{t+1}=\frac{n_k\cdot\mu_k^{t}+n_{k,\mathcal{B}}\cdot\mu_k^{\mathcal{B}}}{n_k+n_{k,\mathcal{B}}}
\end{equation}
where $n_{k}$ represents the number of samples belonging to class $k$ seen by the network until the current update step $t$, $n_{k,\mathcal{B}}$ represents the number of samples belonging to class $k$ in the current batch and $\mu_k^{\mathcal{B}}$ represents the current mini-batch mean vector
relative to the features of class $k$.

Given the class-probability scores in DeepNNO we define the following prediction function:
\begin{equation}
\label{eq:nno-predictiondeep}
k^*=\begin{cases}
      u \in \mathcal{U}_t & \text{if}\ p_k(x) \leq \theta \ \ \ \forall k \in \mathcal{K}_t\\
      \argmax_{k\in\mathcal{K}_t} p_k(x) & \text{otherwise}
    \end{cases}
\end{equation}
where $\theta$ is a threshold which, similarly to the parameter $\tau$ in Eqn.(\ref{eq:nno-score}), regulates the number of samples that are assigned to a new class. While in \cite{bendale2015towards} $\tau$ is a user defined parameter which is kept fixed, in this paper we argue that a better strategy is to dynamically update $\theta$ since the feature extractor function and the mean vectors change during training. {Intuitively, %These parameters allow high flexibility on the design of the model, managing the trade-off between precision and recall.%  Intuitively, $\tau$ is estimated as the average score given to the correct class mean vector within the training set. %Notice that $\tau$ could also be class specific, but we leave this analysis to future works.
while training the deep network, an estimate of $\theta$ can be obtained by looking at the probability score given to the ground truth class. If the score is higher than the threshold, the value of $\theta$ can be increased. Oppositely, the value of the threshold is decreased if the prediction is rejected. Specifically, given a mini-batch $\mathcal{B}$ we update $\theta$ as follows:
\begin{equation}
\label{eq:deep-nno-tau-update}
\theta^{t+1}=\frac{1}{t+1}\left(t\cdot\theta^t+\frac{1}{C_\mathcal{B}}\sum_{k\in\mathcal{K}_t}\bar{p}_{k,\mathcal{B}}\right)
\end{equation}
where % $\theta_{\mathcal{B}}=\frac{1}{C_\mathcal{B}}\sum_{k\in\mathcal{K}_t}\bar{p}_{k,\mathcal{B}}$, 
$C_\mathcal{B}$ is the number of classes in $\mathcal{K}_t$ represented by at least one sample in $\mathcal{B}$ and $\bar{p}_{k,\mathcal{B}}$ is the weighted average probability score of instances of class $k$ within the batch. Formally we consider:
\vspace{-8pt}
\begin{equation}
\label{eq:deep-nno-tau-batch-avg}
\bar{p}_{k,\mathcal{B}}=\frac{1}{\eta_{\mathcal{B},k}}\sum_{i=1}^{\text{b}}w_{k,i}\cdot p_{k}(x_i)
\vspace{-4pt}
\end{equation}
where $\eta_{\mathcal{B},k}=\sum_{i=1}^\text{b} w_{k,i}$ is a normalization factor and:
\begin{equation}
\label{eq:nno-ws}
w_{k,i}=\begin{cases}
     w^+ & \text{if}\ k_i=k \wedge p_k(x_i)>\theta \\
     w^- & \text{if}\ k_i=k \wedge p_k(x_i)\leq \theta \\
      0 & \text{otherwise}
    \end{cases}
\end{equation}
where $w^-$ and $w^+$ are scalar parameters which allow to assign different importance to samples for which the scores given to the ground truth class are respectively rejected or not by the current threshold $\theta$. 

%\mathds{1}_{d_i=j}\
}






%\massi{Under the obtained formulation of $\tau$, an instance $x$ is rejected as a member of class $k$ if $p_k(x)\leq\tau$: consequently an instance belongs to a novel class if it is rejected by all the known classes (\ie $p_k(x)\leq\tau\,\,\,\forall k \in \mathcal{K}_t$).}
To train the network, we employ standard SGD optimization, minimizing the binary cross entropy loss over the training set:
\begin{equation}
\vspace{-8pt}
 \mathcal{L}=\frac{1}{|\mathcal{T}_t|}\sum_i\ell^{\text{cl}}(x_i,k_i) 
 \vspace{-5pt}
\end{equation}
where:
\begin{equation}
 \ell^{\text{cl}}(x_i,k_i) =  \log p_{k_i}(x_i) + \sum_{k \in \mathcal{K}_t} \mathds{1}_{k\neq k_i} \log \left(1 - p_k(x_i)\right)
\end{equation}
After computing the loss, we use standard backpropagation to update the network parameters $\Theta$. After updating $\Theta$, we use the samples of the current batch to update both the class mean estimates $\mu_k$ and the threshold $\theta$, 
using Eqn.\eqref{eq:deep-nno-means} and Eqn.\eqref{eq:deep-nno-tau-update} respectively.  


To allow for incremental learning of our deep network, we exploit two additional components. The first is a memory which stores the most relevant samples of each class in $\mathcal{K}_t$. The relevance of a sample $(x,k)$ is determined by its distance $d_k(x)$ to the class mean $\mu_k$ \ie the lower is the distance, the higher is the relevance of the sample. The memory is used to augment the training set $\mathcal{T}_{t+1}$, allowing to update the mean estimates of the classes in $\mathcal{K}_t$ as the network is trained using samples of novel ones. In order to avoid an unbounded growth, the size of the memory is kept fixed and it is pruned after each incremental step to make room for instances of novel classes. The pruning is performed by removing, for each class in $\mathcal{K}_t$, the instances with lowest relevance}. 

The second component is a batch sampler 
which makes sure that, independently from the size of the memory, a given ratio of the batch is composed by samples taken from the memory. This allows to avoid 
biasing the incremental learning procedure towards novel categories, in the case their number of samples is much larger than the memory size. {Additionally, we add a distillation loss \cite{hinton2015distilling} which act as regularizer and %, at the same time, 
 avoids the forgetting of previously learned features.} Denoting as $\phi_\Theta^{\mathcal{K}_{t-1}}$ the network trained on the set of known classes, the distillation loss is defined as:
\begin{equation}
\ell^{\text{distill}}(x_i) =||\phi_\Theta(x_i)- \phi_\Theta^{\mathcal{K}_{t-1}}(x)||
\end{equation}
The overall loss is thus defined as:
\begin{equation}
\label{eq:il-loss}
 \mathcal{L}=\frac{1}{|\mathcal{T}_t|}\sum_i \left( \ell^{\text{cl}}(x_i,k_i) + \lambda \ell^{\text{distill}}(x_i) \right)
\end{equation}%or biasing too much towards old samples 
where $\lambda$ is an hyperparameter balancing the contribution of $\ell^{\text{distill}}$ within $\mathcal{L}$.%in the opposite case.


%From the way NCM is extended to its deep counterpart, it is straight forward to think about how NNO can be used to train deep CNN, keeping in mind that we
%must estimate not only the class means $\mu_j$ but also the threshold $\tau$. 

\subsubsection{Web-aided OWR}
\label{sec:web-download}
A restricting assumption of the traditional NNO algorithms in \cite{bendale2015towards,de2016online} is that data and labels of unknown classes are made available to the model by an oracle.
%or a preloaded database. 
In practice, especially in robotics applications, this assumption is highly unrealistic since: i) the labels of samples of unknown categories are, by definition, unknown; 
ii) images of the unknown classes for incrementally updating the model are usually unavailable, since it is impossible to have a preloaded 
database containing all possible classes existing in the real world. In this work, we define a general pipeline to address the aforementioned issues.
%In particular, we implement a simple solution for the second problem, while proposing a partial solution for the first one. 
To this extent, we exploit standard search tools used by humans. First, once an object is recognized as unknown, we query the Google Image Search engine\footnote{https://images.google.com/} to retrieve the closest keyword to the current image. Obviously the retrieved label might not be correct \eg due to low resolution of the image or a non canonical pose of the object. Here we tackle this issue through an additional human verification step, %a human operator to correct the label in case of a wrong retrieval, 
leaving the investigation of this problem to future works. As a final step, we use the retrieved keyword to automatically download images from the web. These images represent new training data for the novel category which can be used to incrementally train the deep network. %TODO\massi{Surely there most be some references here. We have both done similar things to this since CogX although not at this scale and maybe more often to learn about the context of objects such as in "Web mining driven object locality knowledge acquisition for efficient robot behavior"} %However notice that the human intervention may be highly reduced by exploiting \eg multiple views of the object acquired through the robot and/or context-based semantic filtering of the candidate labels through semantic networks (\eg \cite{navigli2012babelnet}): we leave these directions to future works. %To tackle these two issues, we propose to leverage information extracted from the web, exploiting standard search tools used by humans. First, once an object is detected as unknown, we query the Google Image Search engine\footnote{https://images.google.com/} to retrieve the closest keyword to the current image.



%Despite the simplicity of the pipeline, there are two issues to tackle. First, Google Image Search may not give the correct label. While this issue maybe partially addressed by collecting more images of the objects from different poses, in this work we decided to adopt an additional human verification step.

%A second issue is that the images downloaded from the Web are very noisy \cite{massouh2017learning}: given a keyword we may end up downloading images whose content does not relate with the novel class. To address this problem, we propose to assign different weights to novel samples in the incremental learning procedure. When a sample is recognized as belonging to a novel class, it is adopted as a reference image. By collecting additional images from the web, the mean vector associated to the novel class is initialized using the corresponding image features. %\massi{Consequently, we can weight the importance of each web sample looking at its distance to the class mean initialized with the real-world images. Denoting the mean of a novel class $k_n$ as $\mu^{\text{R}}_{n}$, a web image $x$ of class $k_n$ will produce a loss:
% \begin{equation}
% \ell^{\text{WEB}}(x,k_n) = \frac{1}{\eta_\ell}\exp\left(-\frac{1}{2}||\phi_\Theta(x) - \mu^{\text{R}}_n ||\right)
% \end{equation}
% which is \eqref{eq:il-loss} weighted by the distance of the sample to the class mean obtained through real images, with $\eta_\ell$ denoting a normalization factor ensuring that, inside a batch, the sum of weights assigned to samples of novel classes still respect the batch sampler ratio previously defined.}. Notice that the same weighting strategy can be applied to the update of the class mean $\mu_{k_n}$ and to the threshold $\tau$. We will analyze the impact of these choices in the experimental section.
